CRADL: Contrastive Representations for Unsupervised Anomaly Detection and Localization

Unsupervised anomaly detection in medical imaging aims to detect and localize arbitrary anomalies without requiring annotated anomalous data during training. Often, this is achieved by learning a data distribution of normal samples and detecting anomalies as regions in the image which deviate from this distribution. Most current state-of-the-art methods use latent variable generative models operating directly on the images. However, generative models have been shown to mostly capture low-level features, s.a. pixel-intensities, instead of rich semantic features, which also applies to their representations. We circumvent this problem by proposing CRADL whose core idea is to model the distribution of normal samples directly in the low-dimensional representation space of an encoder trained with a contrastive pretext-task. By utilizing the representations of contrastive learning, we aim to fix the over-fixation on low-level features and learn more semantic-rich representations. Our experiments on anomaly detection and localization tasks using three distinct evaluation datasets show that 1) contrastive representations are superior to representations of generative latent variable models and 2) the CRADL framework shows competitive or superior performance to state-of-the-art.

==> tex_depr/00_abstract.tex <==
% Intro of unsupervised anomaly detection
Unsupervised anomaly detection in medical imaging aims to detect and localize arbitrary anomalies without requiring annotated anomalous data during training. 
% v1
% Unsupervised anomaly detection in medical imaging aims to detect and localize arbitrary anomalies without requiring labels during training. 
% Improve: annotated anomalous data instead of labels
Often, this is achieved by learning a data distribution of normal samples and detecting anomalies as regions in the image which deviate from this distribution.
Most current state-of-the-art methods use latent variable generative models operating directly on the images.
However, generative models have been shown to mostly capture low-level features s.a. pixel-intensities instead of rich semantic features, which also applies to their representations.
We circumvent this problem by proposing CRADL whose core idea is to model the distribution of normal samples directly in the low-dimensional representation space of an encoder which has been trained with a contrastive pretext-task.
% Because such models operate directly on sample space, they tend to primarily encode low-level statistics (like pixel intensities), 
% while having problems capturing fine semantic information within their representations.
%Recent work has shown that representations obtained from a feature extractor trained with a discriminative task are rich in semantic information.
By utilizing the representations of contrastive learning we aim to fix the over-fixation on low-level features and aim to learn more semantic-rich representations. 
% We propose CRADL, a framework for unsupervised anomaly detection and localization consisting of a feature extractor trained with a contrastive pretext-task and a generative model which learns the distribution of representations. 
%This, however, requires labeled datasets - a prerequisite that is often not fulfilled.
% To perform anomaly detection we use the negative-log-likelihood (NLL) of a sample and we show that back-propagating the gradients of the negative log likelihood into the samples can yield pixel-level anomaly scores (anomaly localization).
Our experiments on the task of anomaly detection and localization on three distinct datasets show that 1) the contrastive representations are superior to generative latent variable models and 2) the CRADL framework shows competetive or superior performance to state-of-the-art.
% We show that the quality of these contrastive representations is superior to representations obtained from prior latent variable models in the context of anomaly localization and evaluate the performance on multiple datasets, and demonstrate strong competitive performance.

==> tex_depr/01_introduction.tex <==
The task of anomaly detection is a long-standing task in the medical domain with many diseases being defined by their deviation from what is considered to be normal \cite{ZYTKOWSKI2021100105}.
In medical image analysis detecting and localizing anomalies is therefore also often the general goal.
With powerful deep learning algorithms this task is often tackled using supervised machine learning, which can be extremely effective given that enough diseased cases are avalaible and annotated during the training process \cite{aggarwal2021diagnostic, mckinneyInternationalEvaluationAI2020}.
% Given a specific problem and sufficient annotated training data at hand, supervised machine learning models can be extremely effective at solving this task.
However, most supervised models are not explicitly designed to handle out-of-distribution (OoD) data and thus might struggle to extrapolate the heterogenity of a disease beyond the training distribution \cite{kellyKeyChallengesDelivering2019}. 
As a consequence, each new class of pathology or imaging modality necessitates the creation of new annotated datasets---a process that scales poorly with the large number of existing pathologies and the ever-increasing amount of image acquisition methods.
Unsupervised anomaly detection promises to deliver predictions in the absence of annotated diseased data.
Thus, overcoming the need for cumbersome manual annotations of diseased images, this class of methods could offer a far greater breadth of applications. 
In principle, this can be realized by learning a distribution of healthy samples. Images (or rather some voxels in the images) `deviating' from this distribution are then defined as outliers. The problem of detecting these deviations can be posed as an Out-of-Distribution (OoD) detection problem similar to the statistical test underlying  blood tests using reference ranges \cite{bainDacieLewisPractical2017}.
% \footnote{https://www.nhlbi.nih.gov/health/blood-tests}.
Specifically in the medical imaging domain, the current state-of-the-art methods for anomaly detection are latent variable generative models operating directly on image space, mainly different subtypes of and scoring methods based on Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs) \cite{baurAutoencodersUnsupervisedAnomaly2020,chenUnsupervisedLesionDetection2020a,schleglFAnoGANFastUnsupervised2019}.
It has been shown, however, that the likelihoods of generative models tend to focus on low-level features such as background characteristics % such as pixel intensities
% \cite{zimmererHighLowlevelImage2019}
\cite{nalisnickDeepGenerativeModels2019,renLikelihoodRatiosOutofDistribution2019,xiaoLikelihoodRegretOutofDistribution2020,meissen2021challenging} and that their representations have problems capturing semantic information \cite{nalisnickDeepGenerativeModels2019,zimmererContextencodingVariationalAutoencoder2018a}. 
Therefore the anomaly scores of these methods built on their likelihoods and representations  are heavily dependent on the aforementioned characteristics not capturing fine semantic information. %  general pixel intensities.

\textit{
Driven by the hypothesis that more discriminative semantic features are superior to low-level features, we investigate if the representations obtained with self-supervised contrastive learning can aid unsupervised anomaly detection and localization.}

For this, we propose CRADL, a simple unsupervised representation-based OoD framework consisting of a generative model working on the representations of a feature extractor, trained in a self-supervised fashion based on SimCLR \cite{chenSimpleFrameworkContrastive2020}.

Our experimental results testing its capabilities and comparing it with state-of-the-art generative latent methods on MRI-Brain lead to the following findings:
\begin{itemize}
    \item Simple generative models s.a. Gaussian Mixture Models and small Normalizing Flows, using the contrastive representations of CRADL lead to state-of-the-art anomaly detection.
    \item Back-propagating the negative log-likelihood (NLL) of CRADL onto a samples allows for state-of-the-art anomaly localization.
    \item The representation based approach can be extended to latent-generative models potentially improving anomaly detection and localization.
    \item Representations obtained with the self-supervised task of CRADL improve upon latent generative represenations for anomaly detection and localization tasks.
\end{itemize}

% Old Detailed contributions
% The semantically rich and low dimensional representations of a feature extractor trained with a contrastive self-supervised task \cite{chenSimpleFrameworkContrastive2020} allow to fit a wide variety of simple generative models such as Gaussian Mixture Models (GMMs). 
% We show that anomalies can be localized by back-propagating the negative log-likelihood of representations into the sample. 
% Finally, in our experimental evaluation, we observe for both anomaly detection and localization competitive performance of CRADL to state-of-the-art methods like the VAE and context encoding VAE and find that the representations of CRADL can yield improvements over reconstruction-based representations for anomaly localization.
% Important add task of MRI brain scan anomaly localization!


% Finally, in our experimental evaluation, we find that the representations of CRADL can yield improvements over reconstruction-based representations for anomaly localization. 


% In this work, we propose CRADL, a simple unsupervised representation-based OoD framework consisting of a feature extractor and a generative model. These semantically rich and low dimensional representations obtained with a feature extractor trained with a contrastive self-supervised task \cite{chenSimpleFrameworkContrastive2020} allow to fit a wide variety of generative models such as Gaussian Mixture Models and Normalizing Flows in a very short time. We show that anomalies can be localized by back-propagating the negative log-likelihood of representations into the sample. Finally, we show in our experimental evaluation  that the representations of our feature can yield improvements over reconstruction-based representations for anomaly localization, show competitive performance.

% In this work, we propose CRADL, a simple unsupervised representation-based OoD framework consisting of a feature extractor and a generative model. These semantically rich and low dimensional representations obtained with a feature extractor trained with a contrastive self-supervised task \cite{chenSimpleFrameworkContrastive2020} allow to fit a wide variety of generative models such as Gaussian Mixture Models and Normalizing Flows in a very short time. We show that anomalies can be localized by back-propagating the negative log-likelihood of representations into the sample. Finally, in our experimental evaluation, we find that the representations of CRADL can yield improvements over reconstruction-based representations for anomaly localization and show competitive performance to state-of-the-art methods like the VAE and context encoding VAE.

%In summary, our contributions are: (1) we investigate contrastive learning for anomaly localization (2) we use SimCLR with GMMs in the OoD context, (3) we use the gradients of a “not-VAE” model (but rather a composite model) to identify anomalies, giving a valid alternative to reconstruction based approaches.
% what is main contribution
% Our main contributions is CRADL:
% % 
% In our experiments on Anomaly Detection and Localization on MRI brain scans, we show the following:
% \begin{itemize}
%     \item CRADL has superior anomaly detection performance 
%     \item CRADL has superior anomaly localization performance
%     \item Self-Supervised representations are more meaningful than latent-variable generative models
% \end{itemize}
The remainder of this work is structured as follows: In section \ref{s:improved-task}, we give a brief task description and state the thought process based on the literature landscape motivating the use of representations for anomaly detection. 
% In section \ref{s:methods} we give an in depth description of the key concepts of representation based anomaly detection and localization. 
In section \ref{s:methods} we detail the way CRADL obtains and uses representations allowing for anomaly detection and localization.
Following this description, we give our experimental details in section \ref{s:expsetup} and set the results into context of our improvements.
% followed by a reflection on the evaluation protocol in section \ref{s:results}. 
Finaly, we conclude the advantages of CRADL in section \ref{s:conclusion} with potential use-cases based on its properties and the results of our experiments.

==> tex_depr/02_relworks.tex <==
\subsection{Anomaly Detection \& Localization from an Out-of-Distribution Perspective}
% Ano Localization And Detection: Master Thesis
% Anomaly Detection \& Localization Based on the definitions of Near and Far Ood as well as semantic and non-semantic shifts, it is concluded that anomaly detection on MRI brain scans is more akin to Near OoD than Far OoD detection. This is because instances with pathologies or minor deviations from the norm are supposed to be detected.
% The additional task of anomaly localization, where a pixel/voxel-wise anomaly heatmap of the input is requested, stands in support of this argument. For example, if the inlier distribution is comprised of healthy MRI brain scans and one group of outliers are CT- Scans of the chest, which exact region of the outlier is anomalous? Based on this example, it should be clear that the task of anomaly localization should only be applied when outliers and inliers show strong structural similarities. An example of these shifts and categorization into Far OoD and Anomaly Detection, which we see as Near OoD, can be seen in figure 2.5.

% Task description anomaly Detection Mode Bias
In \textbf{anomaly and OoD detection} we are interested in differentiating between normal samples (inliers) $x$ of a Dataset $\mathcal{D}$, drawn from the underlying distribution $p^*(x)$, and any anomalous samples, termed outliers $x_{\mathrm{ano}}$, which are drawn from a different - but generally unknown - distribution $Q(x)$.
In OoD detection differentiating between inliers and outliers is commonly tackled by simply defining a score-based binary classifier with the help of a threshold. 
If $Q(x)$ was known exactly, the most straightforward approach would be to define the Bayes Optimal Score
\begin{equation}
   s_B(x) = -\log(\dfrac{p^*(x)}{Q(x)}).
\end{equation}
% Start with unknown Q and strongly dependent on which outliers should be filtered out and in during evaluation one can only test the discriminative on a sub distribrution of Q. 
Generally, however, there is a distinct lack of anomalous samples drawn from $Q(x)$, which is made even more complicated due to the fact that the distribution $Q(x)$ is implicitly defined  by the selection of outliers, which can be done in an arbitrary fashion. E.g. $Q(x)$ can be data stemming from a different dataset, noisy images from the original dataset  or samples containing (previously unknown) classes. \\ 
To circumvent this problem, a common approach is to use the NLL score $s^*(x) = - \log(p^*(x))$ where a generative model is used to approximate the underlying distribution $p(x) \approx p^*(x)$. 
% To circumvent the problem of the generally unkown $Q(x)$ the approach of modeling $p^*(x)$ commonly a measure approximating $s^*(x) = -\log(p^*(x))$ is used by using a generative method $p(x) \approx p^*(x)$. 
This score can then detect outliers based on the assumption that generally: $s(x) \leq s(\hat{x})$ for $x \sim p^*(x)$, $x_{\mathrm{ano}} \sim Q(x)$.
\footnote{In words: the probability of inliers is higher than for arbitrary outliers under the inlier distribution is higher}
% , or in words, that the probability of inliers is higher than for arbitrary outliers under the inlier distribution is higher.
% This however is based on the assumption that meaningful deviations from $p^*(x)$ can be detected by the mean that $s(x) \leq s(\hat{x})$ for $x \sim p^*(x)$, $\hat{x} \sim Q(x)$, or in words that the probability of inliers under the inlier distribution is higher than for the arbitrary outlier distribution. \\
% However, as we will show now by the example of a mixture of Gaussians, that this core assumption can easily break down when $p^*(x)$ consists of multiple modes with different probability mass distributions, or when $Q(x)$ is located inside a high probability region of $p^*(x)$ - making the score unsuitable. 

For \textbf{anomaly localization} one wants to know now which regions of a singular sample $x$ are deviating from normality. 
Based on this task description, the implicit assumption for anomaly localization is that an anomalous sample $x_{\mathrm{ano}}$ is somewhat similar to a normal sample $x_{\mathrm{norm}}$ in a manner where $x_{\mathrm{ano}} = x_{\mathrm{norm}} + a$ where $a$ is the change which makes the sample anomalous.
From an OoD perspective this might be interpreted as raising the question: \textit{If this sample was normal, where would it differ?}
The detection of $a$ is tackled in form of an anomaly heatmap $l(x)$ with the same spatial dimension as $x$ which can either directly be learned, or be based on the OoD detection function $l(x) = \text{Localize}(s(x))$.
The goal of $l(x)$ is to indicate regions of $x_{\mathrm{ano}}$ where $a$ leads to changes from the normal samples and not indicate any regions for normal samples.
% Anomaly Localization is only useful if x_ano is sufficiently close to a normal sample. Essentially it raises the question: If this sample was normal 1) would it be different and 2) where would it differ?


\subsection{Moving from Image Space to Representations}
% Give high-level concept of where to go and why!
% 1. We believe that anomaly detection is most useful for medical imaging if used similarly to medical screenings e.g. bloodtest, but they are done on nice features where fitting a distribution is simple with little anomalies. Features are interpretable and allow localization based on interpretability
% 2. They allow fits based on statistics of many healthy individuals which are relatively easy to acquire (generally most of the population is healthy) since most diseases are classified based on differences of normality.
% 3. No costly annotation of diseased regions etc. to train models.
% We will no discuss the current state in anomaly localization in medical




% Problems of generative models on pixel space
% \paragraph{State-of-the-Art Medical Image Anomaly Detection}
Current state-of-the-art for anomaly detection and localization on medical images are generative methods s.a. VAEs and GANs operating directly in image space. 
The most forward and commonly used approach is the reconstruction difference scoring for both detection and localization \cite{zimmererUnsupervisedAnomalyLocalization2019,baurAutoencodersUnsupervisedAnomaly2020}.
% Move in the right direction
For anomaly detection it has been shown to be advantageous to also use the information in the representation space for anomaly detection \cite{zimmererUnsupervisedAnomalyLocalization2019,zimmererContextencodingVariationalAutoencoder2018a,baur2018deep}.
\citet{baurAutoencodersUnsupervisedAnomaly2020} compared the most common methods based on their anomaly localization capabilities.
They conclude that a VAE-based iterative image restoration setting \cite{chenUnsupervisedLesionDetection2020a} making heavy use of the learned representations performed best across most datasets they evaluated. 
A similar trend has been observed by \citet{zimmererContextencodingVariationalAutoencoder2018a} where they show that the backpropagated loss of the KL-Divergence purely using the representations improved anomaly localization capability.
Other lines of work using VQ-VAEs with discrete latent spaces with spatial information in conjunction with generative models modeling the latent distribution showed 
again that restoration approaches using the represenation space improve anomaly localization performance \cite{pinayaUnsupervisedBrainAnomaly2021,marimont2021anomaly}.
% that actively using the latent space for resampling for anomaly localization improved performance \cite{pinayaUnsupervisedBrainAnomaly2021,marimont2021anomaly}.
\textbf{Take Away:} Actively using the representations of generative models seems to improve the anomaly detection and localization performance of generative methods applied on image space.
% This concept led to us improving
% Move the field of medical anomaly detection closer to SotA OoD in natural imaging by using a scoring measure purely on representations without a reconstructive term. This also falls in line with many medical tests where pre-determined (and meaningful) features are used for anomaly detection based on distribution tests.


\paragraph{General Problems of Generative Models on Image Space}
The image space is high dimensional leading to two natural arising problems of generative models which are the curse of dimensionality which is inherent to probability distributions
\footnote{The curse of dimensionality states that the highest likelihood region in a high dimensional space is basically devoid of samples.}
and the amount of samples needed for a reliable fit of generative model which drastically increases with its complexity and the dimensionality of the distribution.
The distribution of images in the image space, however, is very complex (e.g. non-Gaussian) and is hypothesized to live on a very thin manifold of the whole space.

These properties might be one of the main reasons why it has been shown several times in natural imaging that generative models on pixel space have a hard time detecting samples which are deemed as OoD \cite{nalisnickDeepGenerativeModels2019,nalisnickDetectingOutofDistributionInputs2019}.
% Problem in practice
% Curse of dimensionality
For example, a generative model trained on CIFAR10 gives samples from the SVHN generally a higher likelihood than samples on CIFAR10 \cite{nalisnickDeepGenerativeModels2019,nalisnickDetectingOutofDistributionInputs2019}.
It is hypothesized that this might be due to the curse of dimensionality where SVHN is from a pixel perspective a subset of CIFAR-10 basically subset of CIFAR-10 in the empty high-likelihood region \cite{nalisnickDetectingOutofDistributionInputs2019}.
% Fact of generative Models
% Amount of samples needed for fit of distribution
% Generative models require more training data to reliably fit the distribution of samples with regard to 1) dimensionality of the space in which the samples lie and 2) the DOF the generative model has.
% Concrete example for simplest model: Gaussian
Other works fit a generative model on the low-dimensional representations of supervised classifier showing that even simple generative models allow to reliably solve the aforementioned OoD problem reliably \cite{liangEnhancingReliabilityOutofdistribution2020,leeSimpleUnifiedFramework2018,winkensContrastiveTrainingImproved2020,zhangHybridModelsOpen2020}.
% If now a generative model is fitted on the low-dimensional representations of supervised classifier even simple generative models allow to reliably solve the aforementioned OoD problem reliably \cite{liangEnhancingReliabilityOutofdistribution2020,leeSimpleUnifiedFramework2018,winkensContrastiveTrainingImproved2020,zhangHybridModelsOpen2020}.
\textbf{Take Away:} Lower-dimensional representations carrying meaningful information alleviate inherent problems of generative models on high-dimensional image spaces regarding fit and OoD detection ability.



\paragraph{The Problem of Obtaining and Usefulness of Meaningful Representations}
For standard medical tests e.g. a blood count, meaningful representations to model the distribution of the healthy population are features s.a. hemoglobin and white blood cell levels which are directly read out by a procedure \cite{bainDacieLewisPractical2017}.
For medical imaging and images in general obtaining meaningful features is not as straight-forward.
Deep Learning itself is often seen as a representation learning task and latent variable generative models were historically specifically used to learn useful representations \cite{Goodfellow-et-al-2016}.
Currently, supervised learning is the de-facto standard for  down-stream tasks on images s.a. classification also leading to the best results, but it requires big amounts of annotated training data of each class \cite{chenSimpleFrameworkContrastive2020}. 
As noted in the paragraph above, supervised representations have been shown to work well in the context of OoD with works using generative models on the representations of models trained in supervised fashion.
However, in cases where there is not sufficient annotated training data and/or the task associated with the annotation does not require to capture information potentially crucial information about a sample is lost since injectivity is not per-se a requirement which is a possible explanation for why classifiers are often overconfident for OoD inputs \cite{winkensContrastiveTrainingImproved2020}.
Alternatives would be the latent-space of generative models which, however, have been shown to focus on encoding low-level features s.a. background and color on natural images leading to blurry reconstructions and generations \cite{maaloeBIVAVeryDeep2019}.
Recently Self-Supervised Learning and, more specifically, contrastive learning showed to be able to learn rich semantic representations without requiring label information, by greatly reducing the amount of labeled data to reach fully-supervised down-stream task classification performance, substantially outperforming generative approaches \cite{chenBigSelfSupervisedModels2020,grillBootstrapYourOwn2020}.
\textbf{Take Away:} Self-Supervised learning allows to learn representations without requiring annotated data and leading to better down-stream task performance than current generative models. 
Therefore representations obtained with a contrastive pretext-task have the potential to reduce label-effort compared to a generative pretext task.

% We propose to use a purely self-supervised task inspired by SimCLR to train an encoder to obtain semantically meaningful and rich representations for OoD. 
% This approach is inspired by the works of...



% How do we get better representation?
% Contrastive Learning


% \paragraph{\textbf{Contrastive Learning}} 
% Contrastive Learning can be used to obtain rich semantic representations or to pretrain a model for a specific downstream task.
% This is done by enforcing a clustering of similar data points by pulling together positive pairs (semantically similar data points) while pushing away negative pairs (semantically different data points) in latent space. This can be achieved using the NT-Xent (the normalized temperature-scaled cross-entropy) loss as in SimCLR \citet{chenSimpleFrameworkContrastive2020}. 
% Several Contrastive Training methods have been proposed, mostly differing by the method used to obtain the positive and negative pairs. In the Computer Vision domain, a trend for using data augmentation transformations to obtain these positive and negative pairs has recently emerged \cite{chenSimpleFrameworkContrastive2020,falconFrameworkContrastiveSelfSupervised2020,henaffDataEfficientImageRecognition2020}.
% These methods are commonly used to pretrain the encoder of a classifier with unlabelled data, leading to a significantly reduced amount of labeled data required to train a classifier to a comparable accuracy as a model with access to more labels.
% The representations obtained by these methods allow for better classification than that of Autoencoder-based and many other self-supervised methods, which have historically been used as pretraining for classifiers \cite{chenSimpleFrameworkContrastive2020,falconFrameworkContrastiveSelfSupervised2020,henaffDataEfficientImageRecognition2020}.

% \paragraph{\textbf{Representation-based Out of Distribution detection}}
% Influential works for OoD detection were ODIN \cite{liangEnhancingReliabilityOutofdistribution2020}, the Maximum Softmax Probability \cite{hendrycksBaselineDetectingMisclassified2018}
% as well as \cite{leeSimpleUnifiedFramework2018,hsuGeneralizedODINDetecting2020}.
% These methods were commonly evaluated on far OoD tasks on different datasets, which are not directly translatable to anomaly detection \cite{winkensContrastiveTrainingImproved2020,ahmedDetectingSemanticAnomalies2019}. Another method that only uses the representations in the last encoder layer in combination with Flow-based Deep Generative Models was presented by \citet{zhangHybridModelsOpen2020}.
% \citet{ahmedDetectingSemanticAnomalies2019} demonstrated that a discriminative model which is trained with an additional self-supervised task learns semantically richer representations, leading to better OoD detection. Similarly, \citet{winkensContrastiveTrainingImproved2020} proposed a framework consisting of a discriminative trained classifier with an additional SimCLR inspired task. They used the Mahalanobis distance to fit the distribution of the trained model features, achieving state-of-the-art OoD detection. Concurrently to our work, \citet{sehwag2021ssd} proposed a similar model to \citet{winkensContrastiveTrainingImproved2020} but using a self-supervised task exclusively. While having some conceptual similarities to the approach presented here, they only consider the case of far sample-level OoD. 
 
% \paragraph{\textbf{Generative Models for Medical Anomaly Detection}}
% The current state-of-the-art for image anomaly detection are generative methods such as VAEs and GANs. \citet{baurAutoencodersUnsupervisedAnomaly2020} compared the most common methods based on their anomaly localization capabilities (pixel-level OoD).
% % Where they conclude that the VAE \cite{zimmererUnsupervisedAnomalyLocalization2019} is the most versatile and recommended approach due to the smalles amount of hyperparameters and good performance on all datasets they evaluated on.
% % They show that often reconstruction-based OoD methods such as the VAE show top performance. 
% In their setting, a VAE-based iterative image restoration setting \cite{chenUnsupervisedLesionDetection2020a} performed best across most datasets they evaluated (slightly better than the VAE-based reconstruction difference scoring). 
% However, this iterative restoration is orthogonal to our proposed method and could be directly applied here in analogy to VAEs.
% As such, we chose to use the by \citet{baurAutoencodersUnsupervisedAnomaly2020} recommended latent variable model as baseline: a VAE (due to its performance, simplicity, and optimization).  \citet{chenUnsupervisedLesionDetection2020a} employed a GMVAE for anomaly detection with good results. But despite its architectural similarities to CRADL, we chose only to focus on VAEs as our main baseline, as its performance was shown to be inferior to a VAE while being harder to optimize \cite{baurAutoencodersUnsupervisedAnomaly2020,meissen2021challenging}.
% Recently, different self-supervised approaches, such as context-encoding \cite{zimmererContextencodingVariationalAutoencoder2018a}, image perturbation prediction \cite{li2021cutpaste}, and Multi-Task prediction \cite{venkatakrishnanSelfsupervisedOutofdistributionDetection} have incorporated simple self-supervision tasks in an anomaly-localization framework. Here, we want to continue this line of research but using a two-step approach disentangle the feature learning from the distribution fit and use the recently proposed contrastive pretraining task.  

==> tex_depr/03_methods.tex <==
% Intuition
We propose CRADL, a method using \textit{Contrastive Representations for unsupervised Anomaly Detection and Localization}. 
% Training
Our proposed approach is comprised of two stages as shown in Figure \ref{fig:fit_pipeline}. 
During the first stage, the encoder $f$, which maps a sample $x$ from the image space $X$ to a learned feature/representation space $Z$ : $z=f(x)$, is trained in a self-supervised fashion. 
In the second stage, a generative model $p$ is fitted on the representations of healthy samples, defining the probablity distribution $p(z)$. 
% Score for Ano Detection Sample
The anomaly-score of a sample $x$ is then given by the negative-log-likelihood (NLL) of its representation
\begin{equation}
    s(x) = - \log (p(f(x))).
\end{equation}
% Score for Ano Dection Pixel = Localization
Anomaly localization is then performed using pixel-level anomaly scores (anomaly heatmap) for a sample by back-propagating the gradients of the NLL of the representation of a sample into the image space
\begin{equation}
    l(x) = |\Delta_x -\log(pf(x))|
\end{equation}
Implicitly this approach assumes that regions with large gradients exhibit anomalies.


\begin{figure*}[tb]
    \centering
    \includegraphics[width=.70\textwidth]{figures/full_fig.eps}
    \caption{(a) Visualization of the fitting pipeline, from contrastive pretext (SimCLR) (1) to fitting of the generative model (2). (b) Pixel-wise scores - clamped and normalized for visual inspection.}
    \label{fig:fit_pipeline}
\end{figure*}

\subsection{Contrastive Training}
\label{ss:methods-contrastive}
During the first stage of training CRADL a contrastive pretext-task is used to train the encoder. Since contrastive learning is basically a clustering algortihm, the idea behind the contrastive task is to obtain clusters based on similarity.
The exact contrastive task we use is conceptually identical to SimCLR \cite{chenSimpleFrameworkContrastive2020} while using different data augmentations as transformations.
In SimCLR positive pairs are obtained by using data augmentations $t$ drawn randomly from a set of augmentations $\mathcal{T}$ and negative pairs being all other samples. 
To this end, each sample $x_i$ in a minibatch of $N$ examples is transformed twice, yielding two different views which make up the positive pair. 
The representations produced by feeding the views through the encoder $f$ and projection head $g$, $\tilde{u}_{i} = g(f(\tilde{t}(x_i)))$ and $\hat{u}_{i} = g(f(\hat{t}(x_i)))$, are encouraged to be similar by optimizing the NT-Xent contrastive loss: 
\begin{equation}
    L(x_i) = - \log \dfrac
    {\exp(\text{sim}(\tilde{u}_{i}, \hat{u}_{i}) / \tau)}
    {
    % \exp(\text{sim}(\tilde{u_{i}}, \hat{u_{i}}) / \tau) +
    \sum_{\bar{u} \in \Lambda^{-}} \exp(\text{sim}(\tilde{u}_{i}, \bar{u})) / \tau) }
\end{equation}
Here the set $\Lambda^{-}$ are the negative pairs for sample $x_i$ consists of all examples except $\tilde{u}_i$, which are all other $2N-1$ examples in the minibatch. 
The similarity measure $\text{sim}(x,y)$ is cosine similarity.
The loss over the whole minibatch is then obtained by summing over all positive pairs.


% Data Augmentations?
% \noindent\textbf{Data Augmentations}
% Base Transformations:
% - Resize Transformation
% - Mirror Transformation
% - Spatial Transformation with
% - Brightness Multiplicative Transformation
% Best transformation used for CRADL
% -Random Crop = Base Transformation + Random Cropping (As detailed in Setup)
% With both permutations

\subsection{Generative Model}
\label{ss:methods-generative}
% \paragraph{\textbf{Generative Model}} 
The generative model operating on the representation space to detect and localize anomalies, which is trained in the second stage can be essentially any generative model. In practice, there just needs to be a selection or aggregation criterion.
However, due to the clustered representations of the encoder a `simple' generative models can be used. 
Concretely we decide to use two families which are:
% In general, an arbitrary generative model can be fitted on the representations. 
% GMM part

\noindent\textbf{Gaussian Mixture Model} A Gaussian Mixture Model (GMM) is used, since it is one of the simplest generative models used for anomaly detection. The probability distribution of a GMM with $K$ components is noted in equation \ref{eq:gmm}. We fit the GMM with the Expectation-Maximization (EM) Algorithm \cite{dempsterMaximumLikelihoodIncomplete1977} with $K$ being the number of components (specified before the fit). 
% Gaussian Mixture Model:\\
% - Model is fitted with the Expectation Maximization Algorithm.\\
% - K is the amount of Modes specified before the fit\\
\begin{equation}\label{eq:gmm}
    p(z; \Theta) = \sum_{k=1}^K \mathcal{N}(z; \mu_k, \Sigma_k) \cdot \pi_k
\end{equation}
Here $\mu_k$ is the mean, $\Sigma_k$ is the covariance matrix and $\pi_k$ is the bias of mode $k$.

% Add normalizing flow
\noindent\textbf{Normalizing Flow}
A simple Normalizing flow ($\text{Flow}$) based on the invertible and volume preserving RealNVP architecture \cite{dinhDensityEstimationUsing2017a} is used since it allows to model complex probability distributions.
This is achieved through use of the change of variable formula in combination with a standard normal (Gaussian) $\mathcal{N}(0,\text{I})$ with the same dimensionality as $Z$ as a prior in its latent space 
\begin{equation}
    p(z; \Theta) = \mathcal{N}(\text{Flow}(z); 0, \text{I}) \cdot \left|\det\left( \text{Jacobian}_{\text{Flow}}(z) \right) \right|.
\end{equation}
The normalizing flow should be able to give an upper limit to the performance achievable with GMMs with more components.
% The Normalizing Flow used on the representations of the feature extractor of CRADL is based on the RealNVP architecture (Dinh et al. (2017)) and uses a standard normal (Gaussian) as prior. Since Normalizing Flows allow to fit arbitrary complex distributions, this should allow capturing cases in which the GMMs can not capture the distribution of features. 

% Because the feature space of the encoder is continuous, a small amount of noise $\epsilon$ drawn from a Gaussian distribution is added to each sample in the latent space during the fit. This led to improved stability of the training and lower NLL on the validation set. This approach of data augmentation can be seen as a form of regularizing the flow. 
% TODO: Add change of variable formula



% Ano Localization And Detection: Master Thesis
% Anomaly Detection & Localization Based on the definitions of Near and Far Ood as well as semantic and non-semantic shifts, it is concluded that anomaly detection on MRI brain scans is more akin to Near OoD than Far OoD detection. This is because instances with pathologies or minor deviations from the norm are supposed to be detected.
% The additional task of anomaly localization, where a pixel/voxel-wise anomaly heatmap of the input is requested, stands in support of this argument. For example, if the inlier distribution is comprised of healthy MRI brain scans and one group of outliers are CT- Scans of the chest, which exact region of the outlier is anomalous? Based on this example, it should be clear that the task of anomaly localization should only be applied when outliers and inliers show strong structural similarities. An example of these shifts and categorization into Far OoD and Anomaly Detection, which we see as Near OoD, can be seen in figure 2.5.



% Task Description from Master Thesis:
% In chapter 4.1 the main contribution of this thesis is presented, which is a novel approach for anomaly detection and segmentation. The reimplemented baselines for the comparison with other methods are explained in chapter 4.2. At last, in chapter 4.3 the evaluation of the presented methods for anomaly detection and localization is detailed. All methods presented in this chapter will be used on 2D data such as images. To apply a 2D method on a 3D MRI scan, the scan has to be sliced. This is done in this thesis by taking axial slices, as it is common practice (Baur et al. (2020b); Zimmerer et al. (2018a)). Based on one 2D slice of data x 2 RD⇥D with D as resolution, one score s(x) and one localization l(x) heatmap can be computed. The scoring function s is used to obtain an anomaly scoring for a specific slice:
% s : RD⇥D ! R. (4.1)
% Similarly the localization function l is used to obtain an anomaly scoring for every single
% pixel of the slice:
% l : RD⇥D ! RD⇥D. (4.2)


% Generative Models from Master Thesis:
% Gaussian Mixture Model The GMM is a cluster finding algorithm and generative method, where the amount of clusters is explicitly given as a hyperparameter K. A GMM with K components or clusters has a probability distribution with K modes as noted in equation 2.24. The GMM is fitted with the Expectation-Maximization (EM) Algorithm Dempster et al. (1977), where the number of components K is specified before the fit. This design choice is motivated by the fact that SimCLR and contrastive methods, in general, are clustering algorithms, and GMMs are commonly used to find clusters based on their design (Chen et al. (2020b); Falcon and Cho (2020); He et al. (2020)). Other representation- based OoD methods employ scores based on the shortest Mahalanobis distance of class conditional Gaussians, where the fit is conceptually identical to a GMM with known cluster assignments (Winkens et al. (2020); Lee et al. (2018)).

% Normalizing Flow 
% The Normalizing Flow used on the representations of the feature extractor of CRADL is based on the RealNVP architecture (Dinh et al. (2017)) and uses a standard normal (Gaussian) as prior. Since Normalizing Flows allow to fit arbitrary complex distributions, this should allow capturing cases in which the GMMs can not capture the distribution of features. Because the feature space of the encoder is continuous, a small amount of noise ✏ drawn from a Gaussian distribution is added to each sample in the latent space during the fit. This led to improved stability of the training and lower NLL on the validation set. This approach of data augmentation can be seen as a form of regularizing the flow. More detailed information about Normalizing Flows can be found in chapters 2.3.2 and 3.1.3.
% Add equation for Change of Variable Formula

==> tex_depr/04_expsetup.tex <==
All experiments were performed 3 times with different seeds to obtain a mean and standard deviation which are explicitly state for all experimental results.

\subsection{Datasets}
\label{ss:datasets}
All of our experiments are conducted on T2-weighted MRI brain datasets consisting of 3D medical images.
All datasets are pre-processed similarly with the final step being  image-wise z-score normalization of each image and clipping the intensity from -1.5 to 1.5 following \cite{zimmererContextencodingVariationalAutoencoder2018a}.
For use with our models, the 3D images all slices along the z-axis are used as 2D inputs which are then resized to a resolution of 128x128.
This approach to reduce the complexity of the volumetric data and pre-processing is standard procedure \cite{baurAutoencodersUnsupervisedAnomaly2020, zimmererContextencodingVariationalAutoencoder2018a}
\paragraph{Training Dataset}
For training all of our models we use a subset of the \textbf{HCP} dataset \cite{vanessenHumanConnectomeProject2012}, which purely consists of `normal' MRI Scans, using 894 scans split into training and validation sets.
The HCP dataset consists purely of young and healthy adults taken in a scientific study.
\paragraph{Anomalous Datasets}
We use three anomalous datasets with test and validation sets for score selection to evaluate the anomaly detection and localization performance, all showcasing a 100\% anomaly prevalence per image based on the presence of a tumor or diseased area in the segmentation mask. 
These three datasets are:


\noindent\textbf{HCP Synth.} An artifically created anomalous dataset we created based on the leftover 98 images from the HCP dataset (not used for training) by rendering real-world objects into brain regions as anomalies following the appraoch by \citet{zimmererMedicalOutofDistributionAnalysis2020}.
This allows the test set to have the same original distribution (i.e. population, same scanner, site, registration...) as the training set, with only the anomalies differing. 

\noindent\textbf{ISLES} The ischemic stroke lesion segmentation challenge 2015 (ISLES) dataset \cite{maierISLES2015Public2017} with anomalous regions being the stroke lesions consisting of 28 scans taken from 2 institutions during clinical routine. 
This dataset is explicitly stated to contain different pathologies which are not annotated.

\noindent\textbf{BraTS} The Brain Tumor Segmentation Challenge 2017 (BraTS) dataset \cite{bakasAdvancingCancerGenome2017} with anomalous regions being glioblastoma and lower grade glioma consisting of 286 scans taken from multiple institutions during clinical routine .

To allow better interpretation of our results we give a short dataset-description of with values for interpreting the results for anomaly detection based on slices and anomaly localization based on voxels can be seen in \cref{tab:data_statistics}.

% Redo Table:
% Dataset & Entity 1 & & Entity2..
%  & Val. & Test & Val. & Text &...
% HCP Synth & 
% ISLES
% BraTS
\begin{table}[h!]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cccc|cc}
\toprule
Level      & \multicolumn{2}{c|}{Scans}         & \multicolumn{4}{c|}{Slices}                                                          & \multicolumn{2}{c}{Voxels}                      \\
Value      & \multicolumn{2}{c|}{\# in Dataset} & \multicolumn{2}{c}{\# in Dataset} & \multicolumn{2}{c|}{Anomaly Prevalence} & \multicolumn{2}{c}{Anomaly Prevalence} \\
Dataset    & Test            & Val.            & Test             & Val            & Test                   & Val                    & Test                   & Val                   \\
\midrule
HCP Synth. & 49              & 49              & 7105             & 7105           & 20.5\%                   & 19.8\%                   & 0.649\%                   & 0.770\%                 \\
ISLES      & 20              & 8               & 2671             & 1069           & 36.6\%                   & 34.1\%                   & 1.140\%                   & 1.099\%                 \\
BraTS      & 266             & 20              & 35910            & 2700           & 49.0\%                   & 46.0\%                   & 2.427\%                   & 1.923\% \\
\bottomrule
\end{tabular}
}
        \caption{Statistically relevant characteristics of the anomalous datasets used in our evaluation. The baseline AUPRC of a random score is equal to the prevalence.}
    \label{tab:data_statistics}
\end{table}



% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l|l|l|l}
%          Dataset & Entity & Test & Validation \\
%          \hline
%          HCP Synth. & \#Scans & 49 & 49 \\
%           & \#Slices & 7105 & 7105 \\
%           & Slice prevalence of ano. & 20.54\% & 19.76\%\\
%           & Voxel prevalence of ano. & 0.649\% & 0.770\%\\
%           \hline 
%           BraTS & Scans & 266 & 20 \\
%           & Slices & 35910 & 2700 \\
%           & Slice Prevalence & 49.04\% & 45.95\%\\
%           & Pixel Prevalence & 2.427\% & 1.926\%\\
%           \hline 
%           ISLES & Scans & 20 & 8 \\
%           & Slices & 2671 & 1069 \\
%           & Slice Prevalence & 36.61\% & 34.05\%\\
%           & Pixel Prevalence & 1.140\% & 1.099\%\\
%     \end{tabular}
%         \caption{Description of statistically relevant characteristics of the anomalous datasets used in our evaluation.}
%     \label{tab:data_statistics}
% \end{table}


\paragraph{Distribution Shifts}
There are several distribution shifts from the HCP dataset created for scientific purposes to both clinical datasets ISLES and BraTS leading to different intensity histograms and also prevalences on slice and voxel levels.
Firstly, a population shift is present due to the high prevalence of disease in both clinical datasets which is much higher than that of the whole human population and also often correlated with age of the population. 
Therefore not only unannotated anomalies be present in images from BraTS and ISLES but also structural changes due to different ages of the underlying populations of the datasets.
Secondly, a shift in the images is present due to different scanners which are used for taking the images. Generally the scans for the scientific HCP dataset are taken with a MRI-Scanner with a higher magnetic field strength than used in clinical practice for both BraTS and ISLES.

% This dataset is subject to an age shift compared to HCP due to a generally older population and also exhibits other diseases which are not annotated and might induce changes in the brain structure that could be considered anomalous.

\subsection{Model}
We use a unified model architecture for our experiments which is based on the deep convolutional architecture from \citet{radfordUnsupervisedRepresentationLearning2016}, so our encoder solely consists of 2D-Conv-Layers and our decoder (for the VAE models) of 2D-Transposed-Conv-Layers (for more details, please refer to the Appendix). 
We chose an initial feature map size of 64 and a latent dimension of 512.
For the projection head of CRADL, we use a simple 2-layer MLP with ReLU non-linearities, a 512 dim. hidden layer, and 256 dim. output.
We performed for both our baselines as well as our proposed method experiments with different bottleneck sizes, and feature map counts.\\

% Additional experiments for the pretext model were performed with ResNet18 and ResNet50 architecture, but the DC-Encoder proved to be superior in terms of convergence speed and downstream task performance.\\

\subsection{Training CRADL}
\paragraph{Contrastive PreText-Task}
The contrastive pretext training of the encoder is performed for 100 epochs on the HCP training set using the Adam Optimizer, a learning rate of 1e-4, Cosine Annealing \cite{loshchilovSGDRStochasticGradient2017}, 10 Warm-up Epochs and a weight decay of 1e-6, the temperature of the contrastive loss is 0.5 \cite{chenSimpleFrameworkContrastive2020}.
The encoder for later evaluation is selected based on the smallest loss on the HCP validation set.
As transformations for generating different views for the contrastive task, we use a combination of random cropping, random scaling, random mirroring, rotations, and multiplicative brightness, and Gaussian noise.
\paragraph{Generative Model}
We fit a batch of GMMs with $K\in\{1,2,4,8\}$ on representations of the encoder from all samples in the HCP training set without any augmentation. The means of the components are randomly initialized, and the convergence limit for the EM algorithm is set to $0.1$.
In the Appendix, we present the performance of CRADL with relation to K. 

The Normalizing Flow is also trained on the representation space in the same manner as the GMM to maximize the likelihood of the samples \cite{dinhDensityEstimationUsing2017a}.
All further information regarding the exact training process and model architecture are shown in the Appendix.

We pick the optimal generative model based on a small validation set where we observe the best AUPRC score for anomaly detection and localization. 
% We believe this is a clinically very reasonable approach since the fit of the GMM takes only 10 minutes on a GPU compared to more than 8 hours for the VAE and ceVAE.
We observe in our experiments that best generative model on the HCP dataset does not transfer to the other dataset settings (however, it seems consistent within the same dataset, i.e., between the validation set and test set). This behavior is probably caused by the distribution shifts.

% As a performance measure for the final test sets, we used the pixel-wise AUROC and AUPRC metrics with pixel-level scores, as it is common practice.

\subsection{Baselines}
We train both the VAE and ceVAE for 100 epochs using the Adam Optimizer, a learning rate of 1e-4, and the unified architecture for both encoder and decoder on the HCP training dataset. 
The final models for evaluation are chosen based on the lowest loss on the HCP validation set.
The transformations we use during training of the VAE consisted of random scaling, random mirroring, rotations,  multiplicative brightness, and Gaussian noise, which have shown clear performance improvements in our early experiments. 
For the ceVAE, we add random cutout transformations \cite{zimmererContextencodingVariationalAutoencoder2018a}.  
% The transformation of the VAE are: random mirroring, rotations, and multiplicative brightness augmentations followed by adding additional Gaussian Noise and again clipping to -1.5 to 1.5.
% We experimented with different latent space sizes (128, 512) and the latter had the best OoD performance.\\
% Also for a comparison of the disciminativity of the latent representations we fitted a normalizing flow and multiple gaussian mixture models on the latent representations $\mu$ for a direct comparison between VAE based and our proposed methods.

\subsection{Inference}
We select the best scoring function for CRADL and each baseline and anomalous evaluation dataset based on the best validation set AUPRC metric (see Appendix).
For CRADL the scoring functions are the different generative models on its representations and for the VAE and ceVAE these are the different terms of the loss (Reconstruction difference (Rec.), KL-Divergence, ELBO/combi).
We deem this approach of scoring function selection reasonable and motivate the choice of generative model selection for CRADL by the fact that the fit of all GMMs and the Normalizing Flow on representations take only 50 minutes on one GPU together compared to more than 8 hours for the fit of one VAE or ceVAE.

\paragraph{\textbf{Post-processing of Anomaly Heatmaps}}
%We are mainly interested in the localization of anomalies within the brain. As a performance measure, we used the pixel-wise AUROC and AUPRC metrics with pixel-level scores, as it is common practice. 
% (Scores in this current version are taken on the whole image even though we mask out, following Baur et al.)\\
The post-processing pipeline for the pixel-level scores is identical for all methods evaluated and, based on the approach from \citet{baurAutoencodersUnsupervisedAnomaly2020}, restricted to only use one sample (2D): We zero out all pixel scores outside the brain region. In the next step, 2D median pooling (kernel size=5) is applied to filter out edges and single outliers. As the last step, Gaussian smoothing is applied, inspired by the finding of sparse gradients and convolutional artifacts by \citet{zimmererContextencodingVariationalAutoencoder2018a}. Empirically, also the reconstruction-based scores of the VAE and ceVAE benefited from this step.

\subsection{Evaluation Metrics}
For the two different tasks of anomaly detection and localization, the discriminative power of the scoring function is measured using the Area Under Receiver Operator Curve (AUROC) and Area Under Precision-Recall Curve (AUPRC) due to their independence of a threshold with anomalies being defined as positives.
In our setting, it is more important to detect outliers and a imbalance due to a larger number of healthy slices/voxels than anomalous slices/voxels. Hence, we emphasize the importance of the AUPRC score because it better captures the detection of anomalies.


\noindent For \textbf{anomaly detection}, we aggregate all slices of a dataset and each slice is seen as anomalous if more than 5 voxels are containing an anomaly.


\noindent For \textbf{anomaly localization}, we aggreagte the anomaly heatmaps of all slices and the corresponding ground-truth segmentations.


% \noindent For anomaly detection we aggregate all slices of a dataset and each slice is seen as anomalous if more than 5 voxels are containing an anomaly.

% We chose metrics which directly measure the discriminativity of the scoring function without the need of a threshold.\\
% - Area Under Receiver Operator Curve \\
% - Area Under Precision Recall Curve (Sklearn - Average Precision)  - captures better how well positives/outliers are detected when low prevalence\\


% Master Thesis
% AUPRC
% Area Under Precision-Recall Curve The Area Under Precision-Recall Curve (AUPRC), also known as average precision, is a metric based on the PRC curve similar to the AUROC, which emphasizes the correct classification of positive examples (Davis and Goadrich (2006)). The baseline AUPRC value is the prevalence of the samples, so for a dataset with 10% positives, the baseline AUPRC value corresponds to 0.1 and an AUPRC value of 1 generally marks a perfect classifier. In practice, the AUPRC value is often computed with the average precision method. Commonly used for
% AUROC
% Area Under Receiver Operating Characteristic The Area Under Receiver Operator Characteristic (AUROC) is a metric for discrimination and shows whether a classifier score can rank samples correctly (Davis and Goadrich (2006)). An AUROC score of 0.8 on a dataset means that 80% of the time, the model will return a higher score for condition positive than for condition negative samples. The baseline AUROC value is 0.5, corresponding to a random classifier, whereas an AUROC value of 1 would correspond to a perfect classifier.

==> tex_depr/05_resultsNdiscussion.tex <==
First, we analyze the performance of CRADL for anomaly detection and localization with our re-implementations of the state-of-the-art methods VAE and ce-VAE \cite{baurAutoencodersUnsupervisedAnomaly2020,zimmererContextencodingVariationalAutoencoder2018a} in sections \ref{ss:results-detection} and \ref{ss:results-localization} .
Then, we analyze the discriminative power of the representations obtained with contrastive learning to that of the aforementioned generative models in the context of anomaly detection and localization in \ref{ss:results-representations}.
% First, we analyze the discriminative power of the representations obtained with contrastive learning to that of generative models in the context of anomaly localization and in the next step compare the anomaly localization with the VAE and ceVAE state-of-the-art methods \cite{baurAutoencodersUnsupervisedAnomaly2020, zimmererUnsupervisedAnomalyLocalization2019,zimmererContextencodingVariationalAutoencoder2018a}. 
% Additionally, we compared ourselves with a Flow-based Deep Generative Models (implemented as INN with GLOW-like architecture \cite{kingmaGlowGenerativeFlow2018}), where we show the results in the Supplement. For the results regarding slice-wise OoD detection, we refer to the Supplement as well. 

\subsection{Comparison to State-of-the-Art for Anomaly Detection}
\label{ss:results-detection}
%%%%%%%%%%%%%% SOTA Comparison Table %%%%%%%%%%%%%%
% \begin{table}[]
% \begin{tabular}{ l  r | r | r | r}
%     & & \multicolumn{1}{c|}{CRADL} & \multicolumn{1}{c|}{VAE}  & \multicolumn{1}{c}{ceVAE}  \\

% \hline

% HCP Synth. & AUROC & \bfseries 904(04) & 795(01) & 769(01) \\
%             & AUPRC & \bfseries 788(12) & 492(04) & 436(02) \\

% \hline

% ISLES   & AUROC & 692(04) & 717(02) & \bfseries 727(01) \\
%         & AUPRC & 544(04) & 519(06) & \bfseries 541(01)\\

% \hline

% BraTS   & AUROC &  820(02)& \bfseries 863(01) & \bfseries 863(01) \\
%         & AUPRC &  811(03)& \bfseries 843(01) & \bfseries 843(02) \\
%   \end{tabular}
%     \caption{Slice-wise anomaly detection metrics for different datasets.}
%     \label{tab:detection-results}
% \end{table}


\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{l| rr|rr|rr}
\toprule
Method & \multicolumn{2}{c|}{HCP Synth.} & \multicolumn{2}{c|}{ISLES} & \multicolumn{2}{c}{BraTS} \\
       & \multicolumn{1}{c}{AUPRC}          & \multicolumn{1}{c|}{AUROC}         & \multicolumn{1}{c}{AUPRC}       & \multicolumn{1}{c|}{AUROC}       & \multicolumn{1}{c}{AUPRC}       & \multicolumn{1}{c}{AUROC}       \\
\midrule
CRADL  & \bfseries 77.8(0.7)      & \bfseries 89.8(0.3)     & \bfseries 54.9(0.5)   & 69.3(0.0)   & 81.9(0.2)   & 82.6(0.3)   \\
ceVAE  & 43.2(0.2)      & 76.9(0.1)     & 54.1(0.8)   & \bfseries 72.7(0.1)   & \bfseries 85.6(0.2)   & \bfseries 86.5(0.1)   \\
VAE    & 48.5(0.9)      & 79.4(0.1)     & 51.9(0.6)   & 71.7(0.2)   & 80.7(0.7)   & 83.3(0.6)  \\
\bottomrule
\end{tabular}
}
    \caption{Slice-wise anomaly detection performance. AUROC and AUPRC are given in: mean(standard deviation)\% }
    \label{tab:detection-results}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By comparing CRADL with our re-implementations of the VAE and ceVAE for slice-wise anomaly detection, 
we want to assess the general performance of our approach to that of state-of-the-art baselines.
The results are shown in \cref{tab:detection-results} while all scoring methods of each method are shown in the Appendix.
For the HCP Synth. dataset CRADL substantially outperforms both the VAE and ceVAE. 
% We would like to emphasize that ceVAE with the additional self-supervised context encoding task performs worse on HCP Synth. than the VAE which might stem from a suboptimal additional task for this concrete datset. 
On both ISELES and BRATS the ceVAE is the best performing approach showcasing the advantage of the self-supervised task on ISlES whereas it is tied with the VAE on BraTS.

Due to the aforementioned distribution shifts from the normal (healthy) population on HCP to ISLES and BraTS and the more diverse and subtle set of anomalies on HCP Synth. we conclude therefore that CRADL can capture fine deviations from normality better than a VAE and ceVAE.
And it can be hypothesized that this exact property of CRADL being able to capture fine deviations from normality better than a VAE and ceVAE might be the reason for it performing worst on ISLES and BraTS since based on a distribution perspective essentially all slices from ISLES and BraTs could be considered anomalous.

This hypothesis could also be backed up since for HCP Synth. the best performing scoring methods are based on the GMM with 8 components and the Normalizing Flow which both should be able to capture even relatively complex distributions well, while for ISLES and BraTS the GMM with 1 component leads to the best anomaly detection performance where the latter is not as well suited to capture fine difference in the representation space than the former.

%%%%%%%%%%%%%%%%%%%%% OLD Version %%%%%%%%%%%%%%%%%%%%%%%%
% Here, we compare CRADL with our re-implementations of the state-of-the-art methods VAE and ceVAE, in the context of slice-wise anomaly detection.
% The quantitative results are shown in Table \ref{tab:detection-results}. 
% For the HCP Synth. dataset CRADL achieves the best performance whereas on ISLES and BraTS the VAE and ceVAE both outperform CRADL.
% Based on our 
% However, we would like to emphasize the distribution shifts from HCP to ISLES and BraTS which is further detailed in ...
% Since the distribution of HCP synth is much closer to HCP and all regions which deviate from normality are known we conclude that CRADL can capture fine deviations from normality better than a VAE and ce-VAE.
% This property might lead to the bad performance of ISLES and BraTS since even healthy slices of these datasets might be considered as Outlier based on the HCP dataset.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Why do we show this?

% What are the results

% Insert results

% What do the results show us?


\subsection{Comparison to State-of-the-Art Anomaly Localization}
\label{ss:results-localization}
%%%%%%%%%%%%%% SOTA Comparison Table %%%%%%%%%%%%%%
% \begin{table}[]
% \begin{tabular}{ l  r | r | r | r}
%     & & \multicolumn{1}{c|}{CRADL} & \multicolumn{1}{c|}{VAE}  & \multicolumn{1}{c}{ceVAE}  \\

% \hline

% HCP Synth.& AUROC & \bfseries 978(01) & 951(01) & 921(04) \\
% & AUPRC & \bfseries 288(10) & 210(03) & 172(15) \\

% \hline

% ISLES & AUROC & \bfseries 898(03) & 853(02) & 879(02) \\
% & AUPRC & \bfseries 186(39) & 051(01) & 145(13) \\

% \hline

% BraTS & AUROC & 942(01) & 925(01) & \bfseries 948(03) \\
% & AUPRC & 380(16) & 298(04) & \bfseries 483(03) \\
%   \end{tabular}
%     \caption{Pixel-wise anomaly localization metrics for different datasets.}
%     \label{tab:all_results}
% \end{table}

\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{l| rr|rr|rr}
\toprule
Method & \multicolumn{2}{c|}{HCP Synth.} & \multicolumn{2}{c|}{ISLES} & \multicolumn{2}{c}{BraTS} \\
       & \multicolumn{1}{c}{AUPRC}          & \multicolumn{1}{c|}{AUROC}         & \multicolumn{1}{c}{AUPRC}       & \multicolumn{1}{c|}{AUROC}       & \multicolumn{1}{c}{AUPRC}       & \multicolumn{1}{c}{AUROC}       \\
\midrule
CRADL  & \bfseries 32.5(0.8)      & \bfseries 97.8(0.0)     & \bfseries 18.6 (3.9)  & \bfseries89.8(0.3) & 38.0(1.6)  & 94.2(0.1)  \\
ceVAE  & 17.2(1.5)      & 92.1(0.4)     & 14.5(1.3)  & 87.9 (0.2)  & \bfseries 48.3(3.0)  & \bfseries 94.8(0.3)  \\
VAE    & 24.9(0.6)      & 95.5(0.1)     & 7.7(1.2)   & 87.5 (0.6)  & 29.8(0.4)  & 92.5(0.1) \\
\bottomrule
\end{tabular}
}
    \caption{Voxel-wise anomaly localization performance. AUROC and AUPRC are given in: mean(standard deviation)\% }
    \label{tab:all_results}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The goal behind this experiment is to verify the effectiveness of our approach for anomaly localization by backpropagating gradients of the NLL of generative models operating on a representation space to the image space through an encoder.
To this end, we compare our results again with our state-of-the-art implementations of a VAE and ce-VAE each with three different scores which are reconstruction differencess, backpropagated gradients of the KL-Divergence \cite{zimmererContextencodingVariationalAutoencoder2018a} and the combi-scoring based on a multiplication of KL-Divergence gradients and reconstruction differences \cite{zimmererContextencodingVariationalAutoencoder2018a}.
The results of the best performing anomaly localization scoring methods for CRADl, VAE and ceVAE are shown in \cref{tab:all_results} (the rest is shown in the Appendix).
On HCP Synth. and ISLES CRADL outperforms both VAE and ceVAE. On the BraTS dataset the ceVAE is the best performing method followed by the VAE.
The trend already discussed in \cref{ss:results-detection} continues where HCP Synth. favors for CRADL more complex generative models with the performance increasing for higher values of K.
Interestingly the Normalizing Flow does not perform well, but this might be due to convolutated gradients in the representation space which do not behave as nice as the one of a GMM which approximately scales quadratically with regard to mahalanobis distance from a center. 
The trand that using representations for anomaly localization is advantageous can be observed for the VAE and ceVAE where the combi-score performs best by combining both information from the representation and the prior distribution with the reconstruction error by defining a distribution in image space \cite{zimmererContextencodingVariationalAutoencoder2018a}.  
Further the fact that CRADL performs not as much better on ISLES and worse on BraTS than the ceVAE might be due to the context-encoding task better suited to these dataset where anomalies regions are lesion which often glow bright in T2-weighted MRI scans.

We interpret the strong results on HCP Synth. for anomaly localization showcase that CRADL is capable of localizing anomalies close to the normal distribution and being diverse in appearance (not only bright glowing) better than both ceVAE and VAE.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The quantitative results of our comparison with our state-of-the-art re-implentations are shown in Table \ref{tab:all_results} and qualitative results can be seen in Fig. \ref{fig:fit_pipeline}b. 
% For the HCP Synth. dataset and ISLES-2015, CRADL obtained the best AUROC and AUPRC metrics by a large margin, followed by the presented baselines.
% On the BraTS dataset, the ceVAE outperforms the other methods. However, for the BraTS and ISLES dataset there is a domain gap between the training dataset and test dataset, i.e., different scanners, image quality, and the patients' overall health. This leads to a change in the pixel intensities of the overall pixel distribution. 
% Further, the HCP Synth. dataset includes more varied anomalies and no domain gap and thus its result could receive more importance. 
% Therefore, one could argue that even the brain slices without any pathology could be categorized as OoD (perhaps the anomalous samples are more OoD, but the accuracy of an OoD measurement in the high OoD regions could be considered questionable). 
% On the ISLES-2015 dataset, CRADL shows the best performance, and again, the ceVAE delivers slightly better performance than a reconstruction-based VAE detection.
%%% OPTION 1


\subsection{Anomaly Detection \& Localization with Generative Models on Representation}
\label{ss:results-representations}
\begin{figure}[t]
    \centering
    % \includegraphics[width=.8\textwidth]{figs/reps_comparison.eps}
    \includegraphics[width=\linewidth]{figures/CRADL-Results.pdf}
    \caption{Performance comparison of CRADL with representation based anomaly dection and localization (RADL) on the ceVAE and VAE alongside the KL-Divergence and the best VAE scoring method to assess the performance of purely representation based approaches in general and the advantage of contrastive representations. 
    % -level anomaly localization ($\bar{x} \pm \sigma_x$). We compare features from CRADL (SimCLR + GMM), a ceVAE (VAE + self-supervised context encoding task), a VAE all fitted with a GMM and for both VAE and ceVAE the gradient of the KL-Divergence (see Suppl.).
    }
    \label{fig:representation_comparison}
\end{figure}

This experiment was performed to assess two things with regard to the down-stream tasks of anomaly detection and localization.
Firstly, whether purely purely representation based anomaly scoring for the generative methods VAE and ceVAE offers advantages over standard anomaly scoring.
To this end the same generative models as used for CRADL are fitted in an additional second stage identical to CRADL onto the latent-representations of our VAE and ceVAE implementations (this approach is termed representation based anomaly detection and localization (\textbf{RADL})) and use them for anomaly detection and localization in the same manner as CRADL (see Sec. \ref{ss:methods-generative}).
Secondly, assess whether the contrastive representations of CRADL are better suited for the two aforementioned down-stream tasks than the representations of generative models (generative pretext task)
mothe performance advantage of the con

% the performance of representation obtained with our contrastive pre-text task (CRADL) compared to representations obtained with a generative pre-text task and 2) assess the performance of a purely representation based approach for a VAE and ceVAE.
% For anomaly localization and detection -- what was done?
% To this end the same generative models as used for CRADL are fitted in an additional second stage identical to CRADL onto the latent-representations of our VAE and ceVAE implementations (this approach is termed representation based anomaly detection and localization (RADL)) and use them for anomaly detection and localization in the same manner as CRADL.
% We observe for anomaly detection
% 1. CRADL outperforms all other approaches
% 2. ceVAE and VAE benefit on HCP Synth from this approach! the ceVAE more so than VAE (due to context-encoding task?) -- even over combined scores s,a. elbo and reconstruction
% 3. Trend for HCP for CRADL can be observed on VAE and ceVAE representations too (slightly more complex distributions work well.
% 4. ISLES and BraTS are not as clear but it is often better than pure KL-Divergence except on ISLES

% We observe for anomaly localization
% 1. CRADL outperforms all other approaches see figure except on BraTS
% 2. ceVAE and VAE

% The discriminative power of the representations obtained with CRADL and generative model, here VAE and ceVAE are compared by using GMM on their representations in an identical scheme to CRADL (see Sec. \ref{ss:methods-generative}). 
% To get an estimate of the discriminative power of representations from generative models, in particular VAE and ceVAE, we decided to fit a GMM on their representations in an identical scheme to CRADL (see Sec. \ref{sec:Experiments}). 
% We believe this choice is well-founded because, in theory, the representations of a VAE should be distributed like a unimodal Gaussian. For the VAE models, we additionally compare the gradient of the KL-Divergence, since it also models the feature distribution deviations and is inherent to the model. 
% (to rebut an ``accidental'' better structural fit of the GMM to the contrastive representations in the App. we also show results with a Flow-based generative model).
We depict both anomaly detection and localization performance in Fig. \ref{fig:representation_comparison}, where again the different scoring methods for VAE and RADL are selected based on the best validation set AUPRC value (see Appendix).
Regarding the effectiveness of the purely representation based RADL on the VAE and ceVAE we compare it with the KL-Divergence and the best VAE scoring method selected in sections \ref{ss:results-detection} \& \ref{ss:results-localization}.
For Anomaly Localization it improves the performance over the KL-Divergence on BraTS and on HCP Synth it improves upon the best performing VAE scoring method while underperforming on ISLES. 
For Anomaly Detection the RADL approach leads to substantial performance improvements over the KL-Divergence in all cases except for the ceVAE on BraTS, but it never outperforms the VAE scoring methods also using reconstruction. 

Based on these results we conclude that the RADL approach for generative methods using the representations yields performance benefits over the KL-Divergence and allows to detect fine differences in the distribution as showcased by the results on HCP Synth..

Regarding the second point, assessing our hypothesis regarding performance benefits of the contrastive representations of CRADL, due to carrying more semantic information, compared with generative representations. 
We see our results as strengthening our hypothesis due to the clear performance improvements of CRADL for anomaly localization over the KL-Divergence and RADL approaches for anomaly localization and the performance improvement on HCP Synth. over the ceVAE and VAE performance as well as on ISLES with the exception of the KL-Divergence of the VAE. 
Even though, CRADL has the worst performance on BraTS for anomaly detection is directly counteracting our hypothesis. 
We argue that this might be due to distribution shift which was already mentioned several times and the contrastive representations allow for better detection and localization of fine semantic differences between anomalous and normal brain volumes as the HCP Synth. dataset provides
A further supporting fact of the advantage of a self-supervised pretext task is that the ceVAE, which also employs a self-supervised task, outperforms the VAE.





% , where it becomes apparent that CRADL-based representations outperform both VAE and ceVAE based representations: for both ISLES and HCP Synth. significantly, while on BraTS the KL-Divergence of the ceVAE showed performance within 1 $\sigma$, however with lower mean performance. This strengthens the hypothesis that the self-supervised representations of CRADL carry more semantic information, enabling a better localization of fine semantic differences between anomalous and normal brain volumes. A further supporting fact is that the ceVAE, which also employs a self-supervised task, outperforms the VAE. 
% To verify that the main benefits of CRADL stem from its representations and not purely that the GMM fits the features of SimCLR better than those of a VAE, we also conducted experiments with a Flow-based Deep Generative Models (Real NVP \cite{dinhDensityEstimationUsing2017a}) showing the same trend as for the GMMs. For details on these experiments, we refer the reader to the supplementary material.

\subsection{Caveat of Experimental Setup}
Our experimental evaluations suffers from either being a synthetic problem for HCP synth. or the distribution shifts of BraTS and ISLES discussed in section \ref{ss:datasets}.
We believe that the experimental evidence on HCP synth. is the most trustworthy with regard to the specific task since structural changes due to age and unannotated anomalies in BraTS and ISLES do not allow to showcase performance benefits a certain methods over another.\footnote{Further, it can be observed that tumors and stroke lesion glow bright in T2-weighted MRI-Scans which might give further advantages to methods whose anomaly scores rule can be broken down to: "The more it glows, the more it is anomalous."}

Another critical aspect of the whole field in general is the high prevalence of anomalous cases since this might lead to the possibility of methods being favored in evaluation metrics if giving per-se high scores to certain regions of the brain prone to anomalies (here lesions). This aspect would need to be assessed either directly or evaluated by also having many normal images in the test datasets.

% \noindent Our experimental evaluation also hints towards an evaluation problem which possibly holds back methodological development of anomaly detection and localization approaches in the medical domain which is currently heavily focused on MRI brain scans \cite{baurAutoencodersUnsupervisedAnomaly2020,zimmererContextencodingVariationalAutoencoder2018a,pinayaUnsupervisedBrainAnomaly2021}.
% Evaluating methods on a dataset which exhibits a scan-wise anomaly prevalence of 100\% is problematic since this does not allow to assess whether an anomaly detection approach can succesfully distinguish between anomalous or normal scans which is a major use-case.
% \paragraph{Issue of Evaluation}
% % General Dataset problems, need for 
% \paragraph{Anomaly Detection}

% \paragraph{Anomaly Localization}
% 1. Anomalies are white glowing on T2-Scans BraTS and ISLES

% 2. Post-Processing is OP

% 3. Distribution Shift

% 4. Evaluation Protocol


% Data Shift:
% \paragraph{Data Shift} 
% The three datasets, HCP, BraTS, and ISLES were all acquired by different scanners and not identically pre-processed and co-registered. 
% Thereby, between the normal dataset and BraTS and ISLES is a distribution shift for healthy regions, even after the final step of pre-processing. 
% This distribution shift can be seen, for example, in the intensities of specific brain areas, slightly different orientations of the brain in the scans and intensity histograms (see Suppl.) which all differ. 
% Further there is a distribution shift based on the population in the scans since the HCP scans are healthy young brains whereas BraTS and ISLES mostly consist of diseased patients showcasing a correlation with age. 
% This leads to an age shift from the normal population to the diseased population.
% % Description of histogram
% % The intensities of the HCP, BraTS, and ISLES datasets are visualized in the Supplementary.
% % All three datasets have peaks at intensities -1.5, 0, and 1.5. The peak at intensity 0 is due to the background being set to 0, the other peaks stem from the z-score normalization followed by clipping of the intensities.
% % However, the intensities of the HCP dataset show two additional maxima at intensity values -0.6 and 0.6, whereas BraTS and ISLES only show one at intensity value -0.6. This can be partially explained by the tendency of the pathologies present in the BraTS and ISLES dataset to have very high intensities.


% % Prevalence and Selection Bias
% \paragraph{Selection Bias \& Evaluation} 
% This comes into play due to the fact that the datasets, on which the evaluation is performed (HCP Synth., ISLES, BraTS), have a scan wise prevalence of 100\%.
% Meaning that the whole dataset on which evaluation is performed should be deemed as anomalous due to a tumor or disease being present if seen from an anomaly detection per image perspective.
% This higher than the natural distribution of pathologies and may/does to models giving high scores to specific areas regardeless of the presence of an anomaly having good evaluation metrics due to the computation of metrics on parts (slices/voxels) of the scans, especially AUPRC, AUROC and scores where thresholds are computed directly on the evaluation set, or with a similar distribution. 
% This makes the metrics less interpretable and can lead to a biased evaluation.
% In addition, other pathologies are present on datasets such as ISLES, but these are not always labeled (Maier et al. (2017)). For future experiments it would therefore be advisable to evaluate classification per- formance with thresholds derived on the basis of normal scans in a similar fashion to commonly employed medical scans such as the blood count. This reduces the impact of prevalences in the distribtuion of outliers/pathological data the model is evaluated on.

% % Evaluation Protocol
% The utilization of slice-wise evaluation metrics for anomaly detection and voxel/pixel- wise evaluation metrics for anomaly localization are both subject to biases.
% The slice-wise evaluation metrics are problematic due to the prevalence of anomalies/- pathologies in specific slice regions which was subject of section 6.3.
% While evaluation metrics such as DICE and AUPRC when used pixel or voxel wise are biased towards detecting big anomalies in scans in their scoring. This is because the amount of possible true positives and false negatives for big anomaly is much greater than for one small anomaly.
% Therefore it would be advisable to use a scan-wise evaluation scores for anomaly detection and a metric which better captures the detection of instances of anomalies inside of a scan rather than the segmentation of anomalies.


==> tex_depr/06_conclusion.tex <==
In this work, we propose that propose to purely use representations for unsupervised anomaly detection and localization and investigate to this end contrastive representations of a SimCLR like pretext task. CRADL a simple framework for unsupervised anomaly detection and localization being the result of this investigation. 
% Our experiments on MRI-brain scan datasets clearly show the advantage of using self-supervised representations over the image space to fit a generative model by:

% \noindent Capturing fine differences between inliers and outliers for OoD and anomaly detection and lo

% \noindent Allowing for improved anomaly localization compared to state-of-the-art approaches
% \\ \\

% Lastly the advantage of contrastive representations over generative representations is shown in the context of anomaly detection.



% We show that the representations obtained with this contrastive framework outperform representations obtained with latent variable generative models for anomaly localization.
% Overall CRADL shows competitive anomaly localization performance compared to a VAE and ceVAE. 
% An evident weakness of our approach is the hand-picked selection of the number of components (K) of the GMM, which varies between datasets. However, we suspect for a generative model trained on a representative dataset, minimizing the distribution shift between test and training data, a GMM with multiple components should lead to the best overall performance similar to the HCP Synth. dataset.
% While this work indicated that self-supervision can aid anomaly detection, the often addressed question of the best self-supervised/pretraining task is open to discussion. 
Concretely, we have shown that purely representation based anomaly detection has benefits over generative models operating on image space and that representations of an encoder, trained with a contrastive pretext-task, in combination with a simple generative model, show advantageous properties over generative models on image space leading to better performance in the context anomaly detection and localization. 
This could clearly be observed for fine and diverse differences to the normal distribution.
To this end more powerful generative models like the normalizing flow operating on the representation space seem to perform best for anomaly detection while for anomaly localization simpler generative models like a GMM perform better \footnote{This might be due to the gradients of the NLL for GMMs being more focused towards the maximal likelihoods in representations space.}. 
% A straight-forward and mathematically sound aggregation scheme would be adding up the NLL scores to obtain a score for the whole image.

We see the following two most advantageous case properties of the CRADL approach over generative modeling for anomaly detection and localization:
% Concretely, we have shown here that representations of a SimCLR-like task can show improvements in the context anomaly detection and localization, other tasks \cite{li2021cutpaste,he2021masked} might also be worth investigating.
% the often addressed question of the best self-supervised/pretraining task is open to discussion. 

\noindent - Cases with an Abundance of unannotated healthy and diseased images since the representation learning approach is decoupled from distribution learning. Further it has been shown that using anomalous data for the pretext-task can even be helpful \cite{pinayaUnsupervisedBrainAnomaly2021} for a VQ-VAE.

\noindent -  Cases with a small healthy/normal dataset due the low-dimensionality reducing the amount of samples needed for the fit of the distribution and also simpler generative models compared to generative modeling on image space.

% A big advantage of the SimCLR-like pretext-task is that it does not require labels and can therefore be performed on a dataset consisting of both normal and anomalous images since the representation learning is decoupled from modeling the distribution of normal samples.
% A setting with anomalous samples in the pretext-task dataset might even be beneficial as observed in a similar setting for the VQ-VAE in \cite{pinayaUnsupervisedBrainAnomaly2021} since the representations are then forced to capture the deviations of normality to distinguish between samples for the contrastive task.
% Further, the lower-dimensional representation space allows to fit simple generative models showing good performance.
% We hypothesize that this property should also substantially reduce the amount of normal samples needed compared with purely generative models on pixel-space to A) model the distribution of healthy samples and B) allow for anomaly detection and localization in a similar fashion as it has been shown for supervised classification \cite{chenSimpleFrameworkContrastive2020,grillBootstrapYourOwn2020,he2021masked}.


% Limitations of current methodology
% obtaining representations based on other tasks and their usefulness needs to be evaluated. -- How can self-supervised task be easiliy and fast evaluated?
% Localization method only tested for inputs with 1 channel

% Limitations of our evaluation
% Method has only been shown to work on MRI brain

% Interesting future research direction

% Since the approach of representation based anomaly detection itself is very general as showcased by the experiments in \cref{ss:results-representations}, we believe that other self-supervised tasks \cite{li2021cutpaste,he2021masked} might further increase the performance of CRADL. 
\noindent To increase the potential use-case for the medical domain a generalization to 3D inputs would be necessary and aggregation schemes for cases where a whole needs to be processed in smaller peaces s.a. the slice-wise approach here.
Further, since the approach of representation based anomaly detection itself is very general as showcased by the experiments in \cref{ss:results-representations}, we believe that other self-supervised tasks \cite{li2021cutpaste,he2021masked} might further increase the performance of CRADL. 
Also restorative techniques s.a. image restoration \cite{chenUnsupervisedLesionDetection2020a} or representation resampling \cite{pinayaUnsupervisedBrainAnomaly2021,marimont2021anomaly} might also be incorporated into the CRADL approach.

% Next steps are a generalization to 3D inputs and improve methodology obtaining scores with iterative techniques s.a. image restoration \cite{chenUnsupervisedLesionDetection2020a}.
% As a next step, we believe that using CRADL as prior for an iterative image restoration approach  \cite{chenUnsupervisedLesionDetection2020a} might show further performance improvements.

% A word about the field of anomaly detection and localization in the medical imaging domain

Anomaly detection and localization is a promising research field for the medical imaging domain, due to its potential of alleviating the annotation burden for medical screenings using deep learning to take place while having similar and understood properties to standard medical tests s.a. the blood count.
We hope that our proposed method and insights help push anomaly detection and localization into clinical practice.
